Neural Network Verification with Branch-and-Bound for General Nonlinearities

Branch-and-bound (BaB) is among the most effective techniques for neural network (NN) verification. However, existing works on BaB for NN verification have mostly focused on NNs with piecewise linear activations, especially ReLU networks. In this paper, we develop a general framework, named GenBaB, to conduct BaB on general nonlinearities to verify NNs with general architectures, based on linear bound propagation for NN verification. To decide which neuron to branch, we design a new branching heuristic which leverages linear bounds as shortcuts to efficiently estimate the potential improvement after branching. To decide nontrivial branching points for general nonlinear functions, we propose to pre-optimize branching points, which can be efficiently leveraged during verification with a lookup table. We demonstrate the effectiveness of our GenBaB on verifying a wide range of NNs, including NNs with activation functions such as Sigmoid, Tanh, Sine and GeLU, as well as NNs involving multi-dimensional nonlinear operations such as multiplications in LSTMs and Vision Transformers. Our framework also allows the verification of general nonlinear computation graphs and enables verification applications beyond simple NNs, particularly for AC Optimal Power Flow (ACOPF). GenBaB is part of the latest $\alpha$,$\beta$-CROWN, the winner of the 4th and the 5th International Verification of Neural Networks Competition (VNN-COMP 2023 and 2024). Code for reproducing the experiments is available at https://github.com/shizhouxing/GenBaB.

==> sections/misc.tex <==
\section{Assets}
\label{ap:assets}

We have used the following open-source code repositories and datasets:

\begin{itemize}
\item auto\_LiRPA\footnote{\url{https://github.com/Verified-Intelligence/auto_LiRPA}} under the  BSD-3-Clause license.
\item \abcr\footnote{\url{https://github.com/Verified-Intelligence/alpha-beta-CROWN}} under the  BSD-3-Clause license.
\item The ETH Robustness Analyzer for Neural Networks (ERAN) respository\footnote{\url{https://github.com/eth-sri/eran}} under the Apache-2.0 license, for running DeepPoly and PRIMA.
\item The VeriNet repository\footnote{\url{https://github.com/vas-group-imperial/VeriNet}} with a license provided in the repository\footnote{\url{https://github.com/vas-group-imperial/VeriNet/blob/main/LICENSE.DOCX}}.
\item The Prover repository\footnote{\url{https://github.com/eth-sri/prover}} under the Apache Licence.
\item The DeepT repository\footnote{\url{https://github.com/eth-sri/DeepT}} with unknown liscense.
\item The Softmax bound repository\footnote{\url{https://github.com/NeuralNetworkVerification/bounding-softmax}} with a license provided in the repository\footnote{\url{https://github.com/NeuralNetworkVerification/Marabou/blob/master/COPYING}}.
\item MNIST~\citep{mnist}. License is not clearly known.
\item CIFAR-10~\citep{cifar}. License is not clearly known.
\end{itemize}

\section{Broder Impacts}
\label{sec:impacts}
Our work provides formal guarantees on the properties of neural networks and it takes an important step towards more general and effective neural network verification. We believe it is beneficial for the society by working towards more trustworthy neural networks. We are not aware of any negative social impact.

